The Limit Space of Self-similar Groups and Schreier graphs

The present paper investigates the limit $G$-space $\mathcal{J}_{G}$ generated by the self-similar action of automatic groups on a regular rooted tree. The limit space $\mathcal{J}_{G}$ is the Gromov-Hausdorff limit of the family of Schreier graphs $\Gamma_{n}$; therefore, $\mathcal{J}_{G}$ can be approximated by Schreier graphs on level $n$-th when $n$ tends to infinity. We propose a computer program whose code is written in Wolfram language computes the adjacency matrix of Schreier graph $\Gamma_{n}$ at each specified level of the regular rooted tree. In this paper, the Schreier graphs corresponding to each automatic group is computed by applying the program to some collection of automata groups, including classic automatic groups.

==> ref.tex <==
%% Journal article
@article{barre2007real,
  title={Real and discrete holomorphy: Introduction to an algebraic approach},
  author={Barr{\'e}, Sylvain and Zeghib, Abdelghani},
  journal={Journal de math{\'e}matiques pures et appliqu{\'e}es},
  volume={87},
  number={5},
  pages={495--513},
  year={2007},
  publisher={Elsevier}
}
@article{gromov1999topological,
  title={Topological invariants of dynamical systems and spaces of holomorphic maps: I},
  author={Gromov, Misha},
  journal={Mathematical Physics, Analysis and Geometry},
  volume={2},
  number={4},
  pages={323--415},
  year={1999},
  publisher={Kluwer Academic Publishers}
}
@book{ceccherini2010cellular,
  title={Cellular automata and groups},
  author={Ceccherini-Silberstein, Tullio and Coornaert, Michel},
  volume={36},
  year={2010},
  publisher={Springer}
}
@article{nordin2020orbit,
  title={Orbit growth of Dyck and Motzkin shifts via Artin--Mazur zeta function},
  author={Nordin, Azmeer and Md Noorani, Mohd Salmi and Che Dzul-Kifli, Syahida},
  journal={Dynamical Systems},
  volume={35},
  number={4},
  pages={655--667},
  year={2020},
  publisher={Taylor \& Francis}
}
@article{kesten1959symmetric,
  title={Symmetric random walks on groups},
  author={Kesten, Harry},
  journal={Transactions of the American Mathematical Society},
  volume={92},
  number={2},
  pages={336--354},
  year={1959},
  publisher={JSTOR}
}
@article{grigorchuk1999asymptotic,
  title={On the asymptotic spectrum of random walks on infinite families of graphs},
  author={Grigorchuk, Rostislav I and Zuk, Andrzej},
  journal={Random walks and discrete potential theory (Cortona, 1997)},
  pages={188--204},
  year={1999}
}
@article{grigorchuk2012spectral,
  title={The spectral measure of the Markov operator related to 3-generated 2-group of intermediate growth and its Jacobi parameters},
  author={Grigorchuk, Rostislav Ivanovich and Krylyuk, Ya S},
  journal={Algebra and discrete mathematics},
  number={13,№ 2},
  pages={237--272},
  year={2012},
  publisher={Institute of Applied Mathematics and Mechanics of the National Academy of~…}
}
@article{grigorchuk2021spectra,
  title={Spectra of Cayley graphs of the lamplighter group and random Schr{\"o}dinger operators},
  author={Grigorchuk, Rostislav and Simanek, Brian},
  journal={Transactions of the American Mathematical Society},
  volume={374},
  number={4},
  pages={2421--2445},
  year={2021}
}
@book{nekrashevych2005self,
  title={Self-similar groups},
  author={Nekrashevych, Volodymyr},
  number={117},
  year={2005},
  publisher={American Mathematical Soc.}
}
@article{bartholdi1999spectrum,
  title={On the spectrum of Hecke type operators related to some fractal groups},
  author={Bartholdi, Laurent and Grigorchuk, Rostislav I},
  journal={arXiv preprint math/9910102},
  year={1999}
}
@article{bartholdi2000spectra,
  title={Spectra of non-commutative dynamical systems and graphs related to fractal groups},
  author={Bartholdi, Laurent and Grigorchuk, Rostislav I},
  journal={Comptes Rendus de l'Acad{\'e}mie des Sciences-Series I-Mathematics},
  volume={331},
  number={6},
  pages={429--434},
  year={2000},
  publisher={Elsevier}
}
@book{totaro2014group,
  title={Group cohomology and algebraic cycles},
  author={Totaro, Burt},
  number={204},
  year={2014},
  publisher={Cambridge University Press}
}
@book{bass2006cyclic,
  title={Cyclic renormalization and automorphism groups of rooted trees},
  author={Bass, Hyman and Otero-Espinar, Maria V and Rockmore, Daniel and Tresser, Charles},
  year={2006},
  publisher={Springer}
}
@book{ceccherini2010representation,
  title={Representation theory of the symmetric groups: the Okounkov-Vershik approach, character formulas, and partition algebras},
  author={Ceccherini-Silberstein, Tullio and Scarabotti, Fabio and Tolli, Filippo},
  volume={121},
  year={2010},
  publisher={Cambridge University Press}
}
@article{bekka2016spectral,
  title={Spectral rigidity of group actions on homogeneous spaces},
  author={Bekka, Bachir},
  journal={arXiv preprint arXiv:1602.02892},
  year={2016}
}
@book{figa1991harmonic,
  title={Harmonic analysis and representation theory for groups acting on homogenous trees},
  author={Fig{\`a}-Talamanca, Alessandro and Nebbia, Claudio},
  volume={162},
  year={1991},
  publisher={Cambridge University Press}
}
@article{ceccherini2006trees,
  title={Trees, wreath products and finite Gelfand pairs},
  author={Ceccherini-Silberstein, Tullio and Scarabotti, Fabio and Tolli, Filippo},
  journal={Advances in Mathematics},
  volume={206},
  number={2},
  pages={503--537},
  year={2006},
  publisher={Elsevier}
}
@article{d2009group,
  title={A group of automorphisms of the rooted dyadic tree and associated Gelfand pairs},
  author={D’Angeli, Daniele and Donno, Alfredo},
  journal={Rendiconti del Seminario Matematico della Universit{\`a} di Padova},
  volume={121},
  pages={73--92},
  year={2009}
}
@article{ceccherini2007finite,
  title={Finite Gel’fand pairs and their applications to probability and statistics},
  author={Ceccherini-Silberstein, T and Scarabotti, F and Tolli, F},
  journal={Journal of Mathematical Sciences},
  volume={141},
  number={2},
  pages={1182--1229},
  year={2007},
  publisher={Springer}
}
@article{d2007self,
  title={Self-similar groups and finite Gelfand pairs},
  author={D’Angeli, Daniele and Donno, Alfredo},
  journal={Algebra and Discrete Mathematics},
  year={2007},
  publisher={Інститут прикладної математики і механіки НАН України}
}
@incollection{ceccherini2009finite,
  title={Finite Gelfand pairs: examples and applications},
  author={Ceccherini-Silberstein, Tullio and D'ANGELI, DANIELE and Donno, Alfredo and Scarabotti, Fabio and Tolli, Filippo},
  booktitle={Ischia group theory 2008},
  pages={7--41},
  year={2009},
  publisher={World Scientific}
}
@incollection{bartholdi2003fractal,
  title={From fractal groups to fractal sets},
  author={Bartholdi, Laurent and Grigorchuk, Rostislav and Nekrashevych, Volodymyr},
  booktitle={Fractals in Graz 2001},
  pages={25--118},
  year={2003},
  publisher={Springer}
}
@book{ratcliffe1994foundations,
  title={Foundations of hyperbolic manifolds},
  author={Ratcliffe, John G and Axler, S and Ribet, KA},
  volume={149},
  year={1994},
  publisher={Springer}
}
@book{bridson2013metric,
  title={Metric spaces of non-positive curvature},
  author={Bridson, Martin R and Haefliger, Andr{\'e}},
  volume={319},
  year={2013},
  publisher={Springer Science \& Business Media}
}
@article{bartholdi2006automata,
  title={Automata, groups, limit spaces, and tilings},
  author={Bartholdi, Laurent and Henriques, Andr{\'e} G and Nekrashevych, Volodymyr V},
  journal={Journal of Algebra},
  volume={305},
  number={2},
  pages={629--663},
  year={2006},
  publisher={Elsevier}
}
@book{kigami2001analysis,
  title={Analysis on fractals},
  author={Kigami, Jun},
  number={143},
  year={2001},
  publisher={Cambridge University Press}
}
@article{grigorchuk2011some,
  title={Some topics in the dynamics of group actions on rooted trees},
  author={Grigorchuk, Rostislav I},
  journal={Proceedings of the Steklov Institute of Mathematics},
  volume={273},
  number={1},
  pages={64--175},
  year={2011},
  publisher={Springer}
}
@article{bartholdi1999parabolic,
  title={On parabolic subgroups and Hecke algebras of some fractal groups},
  author={Bartholdi, Laurent and Grigorchuk, Rostislav I},
  journal={arXiv preprint math/9911206},
  year={1999}
}
@article{grigorchuk2018spectra,
  title={Spectra of Schreier graphs of Grigorchuk’s group and Schroedinger operators with aperiodic order},
  author={Grigorchuk, Rostislav and Lenz, Daniel and Nagnibeda, Tatiana},
  journal={Mathematische Annalen},
  volume={370},
  number={3},
  pages={1607--1637},
  year={2018},
  publisher={Springer}
}
@article{grigorchuk2001lamplighter,
  title={The lamplighter group as a group generated by a 2-state automaton, and its spectrum},
  author={Grigorchuk, Rostislav I and {\.Z}uk, Andrzej},
  journal={Geometriae Dedicata},
  volume={87},
  number={1},
  pages={209--244},
  year={2001},
  publisher={Springer}
}
@article{nekrashevych2008groups,
  title={Groups and analysis on fractals},
  author={Nekrashevych, Volodymyr and Teplyaev, Alexander},
  journal={Analysis on graphs and its applications},
  volume={77},
  pages={143--180},
  year={2008},
  publisher={Citeseer}
}
@article{donno2013constructing,
  title={Constructing Laplacians on Limit Spaces of Self-similar Groups},
  author={Donno, Alfredo},
  journal={Trends in Harmonic Analysis},
  pages={245--275},
  year={2013},
  publisher={Springer}
}
@article{grigorchuk2004ihara,
  title={The Ihara zeta function of infinite graphs, the KNS spectral measure and integrable maps},
  author={Grigorchuk, Rostislav I and Zuk, Andrzej},
  journal={Random walks and geometry},
  pages={141--180},
  year={2004},
  publisher={Walter de Gruyter GmbH \& Co. KG Berlin}
}
@article{bondarenko2008classification,
  title={Classification of groups generated by 3-state automata over a 2-letter alphabet},
  author={Bondarenko, Ievgen and Grigorchuk, Rostislav and Kravchenko, Rostyslav and Muntyan, Yevgen and Nekrashevych, Volodymyr and Savchuk, Dmytro and Sunic, Zoran},
  journal={arXiv preprint arXiv:0803.3555},
  year={2008}
}
@incollection{gromov1987hyperbolic,
  title={Hyperbolic groups},
  author={Gromov, Mikhael},
  booktitle={Essays in group theory},
  pages={75--263},
  year={1987},
  publisher={Springer}
}
@article{kapovich2002boundaries,
  title={Boundaries of hyperbolic groups},
  author={Kapovich, Ilya and Benakli, Nadia},
  journal={arXiv preprint math/0202286},
  year={2002}
}
@article{bondarenko2008classification,
  title={Classification of groups generated by 3-state automata over a 2-letter alphabet},
  author={Bondarenko, Ievgen and Grigorchuk, Rostislav and Kravchenko, Rostyslav and Muntyan, Yevgen and Nekrashevych, Volodymyr and Savchuk, Dmytro and Sunic, Zoran},
  journal={arXiv preprint arXiv:0803.3555},
  year={2008}
}
@article{delyon1991recurrence,
  title={Recurrence of the eigenstates of a Schr{\"o}dinger operator with automatic potential},
  author={Delyon, F and Peyriere, J},
  journal={Journal of statistical physics},
  volume={64},
  number={1},
  pages={363--368},
  year={1991},
  publisher={Springer}
}
@incollection{bellissard1992gap,
  title={Gap labelling theorems for Schr{\"o}dinger operators},
  author={Bellissard, Jean},
  booktitle={From number theory to physics},
  pages={538--630},
  year={1992},
  publisher={Springer}
}
@article{avron1981almost,
  title={Almost periodic Schroedinger operators. Pt. 1},
  author={Avron, J and Simon, B},
  journal={Communications in Mathematical Physics},
  volume={82},
  number={1},
  pages={101--120},
  year={1981}
}
@article{simon2008schrodinger,
  title={Schrodinger Operators with Purely Discrete Spectrum},
  author={Simon, Barry},
  journal={arXiv preprint arXiv:0810.3275},
  year={2008}
}
@article{sy1992discrete,
  title={Discrete Schr{\"o}dinger operators on a graph},
  author={Sy, Polly Wee and Sunada, Toshikazu},
  journal={Nagoya Mathematical Journal},
  volume={125},
  pages={141--150},
  year={1992},
  publisher={Cambridge University Press}
}
@incollection{sunada1988fundamental,
  title={Fundamental groups and Laplacians},
  author={Sunada, Toshikazu},
  booktitle={Geometry and analysis on manifolds},
  pages={248--277},
  year={1988},
  publisher={Springer}
}
@article{grigorchuk2018spectra,
  title={Spectra of Schreier graphs of Grigorchuk’s group and Schroedinger operators with aperiodic order},
  author={Grigorchuk, Rostislav and Lenz, Daniel and Nagnibeda, Tatiana},
  journal={Mathematische Annalen},
  volume={370},
  number={3},
  pages={1607--1637},
  year={2018},
  publisher={Springer}
}
@article{grigorchuk2017schreier,
  title={Schreier graphs of Grigorchuk’s group and a subshift associated to a nonprimitive substitution},
  author={Grigorchuk, Rostislav and Lenz, Daniel and Nagnibeda, Tatiana},
  journal={Groups, graphs and random walks},
  volume={436},
  pages={250--299},
  year={2017},
  publisher={Cambridge University Press Cambridge}
}
@article{bondarenko2007post,
  title={Post-critically finite self-similar groups},
  author={Bondarenko, Ievgen and Nekrashevych, Volodymyr},
  journal={arXiv preprint math/0701824},
  year={2007}
}
@article{grigorchuk2020spectra,
  title={On spectra and spectral measures of Schreier and Cayley graphs},
  author={Grigorchuk, Rostislav and Nagnibeda, Tatiana and P{\'e}rez, Aitor},
  journal={arXiv preprint arXiv:2007.03309},
  year={2020}
}
@article{ju2012post,
  title={Post-critically finite fractal and Martin boundary},
  author={Ju, Hongbing and Lau, Ka-Sing and Wang, Xiang-Yang},
  journal={Transactions of the American Mathematical Society},
  volume={364},
  number={1},
  pages={103--118},
  year={2012}
}
@article{bondarenko2011ends,
  title={Ends of Schreier graphs of self-similar groups},
  author={Bondarenko, Ievgen and D’Angeli, Daniele and Nagnibeda, Tatiana},
  journal={preprint},
  year={2011}
}
@article{bondarenko2011graph,
  title={Graph-directed systems and self-similar measures on limit spaces of self-similar groups},
  author={Bondarenko, Ievgen V and Kravchenko, Rostyslav V},
  journal={Advances in Mathematics},
  volume={226},
  number={3},
  pages={2169--2191},
  year={2011},
  publisher={Elsevier}
}
@incollection{bass2001tree,
  title={Tree lattices},
  author={Bass, Hyman and Lubotzky, Alexander},
  booktitle={Tree Lattices},
  pages={25--33},
  year={2001},
  publisher={Springer}
}
@article{bass1992ihara,
  title={The Ihara-Selberg zeta function of a tree lattice},
  author={Bass, Hyman},
  journal={International Journal of Mathematics},
  volume={3},
  number={06},
  pages={717--797},
  year={1992},
  publisher={World Scientific}
}
@article{bass1993covering,
  title={Covering theory for graphs of groups},
  author={Bass, Hyman},
  journal={Journal of pure and applied algebra},
  volume={89},
  number={1-2},
  pages={3--47},
  year={1993},
  publisher={Elsevier}
}
@incollection{serre1979local,
  title={Local class field theory},
  author={Serre, Jean-Pierre},
  booktitle={Local Fields},
  pages={188--203},
  year={1979},
  publisher={Springer}
}
@book{serre2002trees,
  title={Trees},
  author={Serre, Jean-Pierre},
  year={2002},
  publisher={Springer Science \& Business Media}
}
@techreport{gromov1992asymptotic,
  title={Asymptotic invariants of infinite groups},
  author={Gromov, Mikhael},
  year={1992},
  institution={P00001028}
}
@article{gromov1981groups,
  title={Groups of polynomial growth and expanding maps (with an appendix by Jacques Tits)},
  author={Gromov, Michael},
  journal={Publications Math{\'e}matiques de l'IH{\'E}S},
  volume={53},
  pages={53--78},
  year={1981}
}
@inproceedings{gromov1980hyperbolic,
  title={Hyperbolic manifolds, groups and actions},
  author={Gromov, Mikhael},
  booktitle={Riemann surfaces and related topics: Proceedings of the 1978 Stony Brook Conference (State Univ. New York, Stony Brook, NY, 1978)},
  volume={97},
  pages={183--213},
  year={1980}
}
@article{simon2001hausdorff,
  title={Hausdorff dimension of limit sets for parabolic IFS with overlaps},
  author={Simon, K{\'a}roly and Solomyak, Boris and Urba{\'n}ski, M},
  journal={Pacific journal of mathematics},
  volume={201},
  number={2},
  pages={441--478},
  year={2001},
  publisher={Mathematical Sciences Publishers}
}
@article{gel1952geodesic,
  title={Geodesic flows on manifolds of constant negative curvature},
  author={Gel'fand, Izrail Moiseevich and Fomin, Sergei Vasil'evich},
  journal={Uspekhi Matematicheskikh Nauk},
  volume={7},
  number={1},
  pages={118--137},
  year={1952},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian~…}
}
@incollection{anosov2020ergodic,
  title={Ergodic properties of geodesic flows on closed Riemannian manifolds of negative curvature},
  author={Anosov, Dmitry Victorovich},
  booktitle={Hamiltonian Dynamical Systems},
  pages={486--489},
  year={2020},
  publisher={CRC Press}
}
@article{anosov1967geodesic,
  title={Geodesic flows on closed Riemannian manifolds of negative curvature},
  author={Anosov, Dmitry Victorovich},
  journal={Trudy Matematicheskogo Instituta Imeni VA Steklova},
  volume={90},
  pages={3--210},
  year={1967},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian~…}
}
@article{hopf1971ergodic,
  title={Ergodic theory and the geodesic flow on surfaces of constant negative curvature},
  author={Hopf, Eberhard},
  journal={Bulletin of the American Mathematical Society},
  volume={77},
  number={6},
  pages={863--877},
  year={1971},
  publisher={American Mathematical Society}
}
@article{yue1996ergodic,
  title={The ergodic theory of discrete isometry groups on manifolds of variable negative curvature},
  author={Yue, Chengbo},
  journal={Transactions of the American Mathematical Society},
  volume={348},
  number={12},
  pages={4965--5005},
  year={1996}
}
@article{jezouin2013quantum,
  title={Quantum limit of heat flow across a single electronic channel},
  author={Jezouin, S{\'e}bastien and Parmentier, FD and Anthore, A and Gennser, U and Cavanna, A and Jin, Yong and Pierre, F},
  journal={Science},
  volume={342},
  number={6158},
  pages={601--604},
  year={2013},
  publisher={American Association for the Advancement of Science}
}
@article{bourgain2003entropy,
  title={Entropy of quantum limits},
  author={Bourgain, Jean and Lindenstrauss, Elon},
  journal={Communications in mathematical physics},
  volume={233},
  number={1},
  pages={153--171},
  year={2003},
  publisher={Springer}
}
@article{anantharaman2007entropy,
  title={Entropy and localization of eigenfunctions},
  author={Anantharaman, Nalini},
  journal={S{\'e}minaire {\'E}quations aux d{\'e}riv{\'e}es partielles (Polytechnique) dit aussi" S{\'e}minaire Goulaouic-Schwartz"},
  pages={1--17},
  year={2007}
}
@article{bishop1997hausdorff,
  title={Hausdorff dimension and Kleinian groups},
  author={Bishop, Christopher J and Jones, Peter W},
  journal={Acta Mathematica},
  volume={179},
  number={1},
  pages={1--39},
  year={1997},
  publisher={Institut Mittag-Leffler}
}
@article{d2009schreier,
  title={Schreier graphs of the Basilica group},
  author={D'angeli, Daniele and Donno, Alfredo and Matter, Michel and Nagnibeda, Tatiana},
  journal={arXiv preprint arXiv:0911.2915},
  year={2009}
}
@incollection{d2011partition,
  title={Partition functions of the Ising model on some self-similar Schreier graphs},
  author={D’Angeli, Daniele and Donno, Alfredo and Nagnibeda, Tatiana},
  booktitle={Random walks, boundaries and spectra},
  pages={277--304},
  year={2011},
  publisher={Springer}
}
@article{aleshin1972finite,
  title={Finite automata and Burnside's problem for periodic groups},
  author={Aleshin, Stanislav V},
  journal={Mathematical Notes of the Academy of Sciences of the USSR},
  volume={11},
  number={3},
  pages={199--203},
  year={1972},
  publisher={Springer}
}
@book{margulis1991discrete,
  title={Discrete subgroups of semisimple Lie groups},
  author={Margulis, Gregori A},
  volume={17},
  year={1991},
  publisher={Springer Science \& Business Media}
}
@article{lenz2002uniform,
  title={Uniform ergodic theorems on subshifts over a finite alphabet},
  author={Lenz, Daniel},
  journal={Ergodic Theory and Dynamical Systems},
  volume={22},
  number={1},
  pages={245--255},
  year={2002},
  publisher={Cambridge University Press}
}
@article{lavrenyuk2008lattice,
  title={Lattice of normal subgroups of a group of local isometries of the boundary of a spherically homogeneous tree.},
  author={Lavrenyuk, Ya V and Sushchanskii, VI},
  journal={Ukrainian Mathematical Journal},
  volume={60},
  number={10},
  year={2008}
}
@book{lindstrom1990brownian,
  title={Brownian motion on nested fractals},
  author={Lindstrom, Tom and Lindstr{\o}m, Tom},
  number={420},
  year={1990},
  publisher={American Mathematical Soc.}
}
@article{bowditch1998topological,
  title={A topological characterisation of hyperbolic groups},
  author={Bowditch, Brian},
  journal={Journal of the American Mathematical Society},
  volume={11},
  number={3},
  pages={643--667},
  year={1998}
}
@article{-1994,
doi	= {10.1515/crll.1994.455.57},
title	= {Ergodicity of harmonic invariant measures for the geodesic flow on hyperbolic spaces.},
journal	= {Journal für die reine und angewandte Mathematik (Crelles Journal)    1994-oct 01 vol. 1994 iss. 455},

year	= {1994},
month	= {oct},
day	= {01},
volume	= {1994},
issue	= {455},
page	= {57--104},
url =       {libgen.li/file.php?md5=50f6bc9a48d265b20890a72bf2c420af},
}
